Search for interacting galaxy clusters from SDSS DR-17 employing optimized friend-of-friend algorithm and multi-messenger tracers

In the theoretical framework of hierarchical structure formation, galaxy clusters evolve through continuous accretion and mergers of substructures. Cosmological simulations have revealed the best picture of the Universe as a 3-D filamentary network of dark-matter distribution called the cosmic web. Galaxy clusters are found to form at the nodes of this network and are the regions of high merging activity. Such mergers being highly energetic, contain a wealth of information about the dynamical evolution of structures in the Universe. Observational validation of this scenario needs a colossal effort to identify numerous events from all-sky surveys. Therefore, such efforts are sparse in literature and tend to focus on individual systems. In this work, we present an improved search algorithm for identifying interacting galaxy clusters and have successfully produced a comprehensive list of systems from SDSS DR-17. By proposing a set of physically motivated criteria, we classified these interacting clusters into two broad classes, 'merging' and 'pre-merging/postmerging' systems. Interestingly, as predicted by simulations, we found that most cases show cluster interaction along the prominent cosmic filaments of galaxy distribution (i.e., the proxy for DM filaments), with the most violent ones at their nodes. Moreover, we traced the imprint of interactions through multi-band signatures, such as diffuse cluster emissions in radio or X-rays. Although we could not find direct evidence of diffuse emission from connecting filaments and ridges; our catalogue of interacting clusters will ease locating such faintest emissions as data from sensitive telescopes like eROSITA or SKA, becomes accessible

==> tables/merging.tex <==
\multirow{3}{*}{M1}&0.597&0.535&0.08&19.0&50.209&0.573&1.033&0.616&0.553&0.08\\&0.729&0.944&0.08&50.0&47.92&1.56&7.643&0.726&0.859&0.08\\&0.808&1.07&0.079&30.0&54.784&0.828&2.156&0.786&1.054&0.079\\\hline
\multirow{2}{*}{M2}&4.508&0.491&0.018&10.0&28.513&0.242&0.184&4.58&0.48&0.018\\&5.12&0.826&0.018&19.0&66.216&0.198&0.123&5.125&0.764&0.018\\\hline
\multirow{2}{*}{M3}&11.251&0.965&0.124&23.0&46.116&1.479&6.868&11.243&1.022&0.124\\&11.252&0.953&0.124&20.0&48.733&1.216&4.645&11.254&0.973&0.124\\\hline
\multirow{2}{*}{M4}&13.517&0.994&0.043&26.0&59.225&0.484&0.735&13.594&0.995&0.043\\&13.564&0.994&0.043&27.0&57.23&0.519&0.846&13.603&1.003&0.043\\\hline
\multirow{2}{*}{M5}&14.418&0.403&0.08&12.0&27.334&0.659&1.364&14.431&0.387&0.08\\&14.452&0.382&0.08&13.0&27.141&0.718&1.619&14.452&0.385&0.08\\\hline
\multirow{2}{*}{M6}&16.83&14.253&0.075&32.0&109.311&0.395&0.489&16.834&14.26&0.075\\&16.834&14.249&0.075&34.0&107.632&0.426&0.569&16.841&14.252&0.075\\\hline
\multirow{2}{*}{M7*}&17.518&15.799&0.061&10.0&64.918&0.289&0.263&17.509&15.776&0.061\\&17.519&15.758&0.06&12.0&61.098&0.369&0.428&17.525&15.745&0.06\\\hline
\multirow{2}{*}{M8*}&18.036&15.729&0.061&26.0&97.039&0.502&0.793&18.01&15.693&0.061\\&18.075&15.739&0.061&19.0&132.174&0.27&0.229&18.06&15.747&0.061\\\hline
\multirow{2}{*}{M9}&18.531&0.792&0.065&19.0&32.871&0.88&2.432&18.488&0.799&0.065\\&18.534&0.803&0.065&15.0&33.258&0.689&1.491&18.563&0.833&0.065\\\hline
\multirow{2}{*}{M10}&18.76&0.297&0.045&163.0&197.6&0.759&1.809&18.738&0.325&0.045\\&19.149&0.581&0.045&11.0&24.945&0.401&0.504&19.121&0.622&0.045\\\hline
\multirow{2}{*}{M11*}&18.782&15.349&0.068&13.0&51.938&0.453&0.643&18.776&15.353&0.068\\&18.783&15.345&0.068&11.0&48.241&0.412&0.534&18.799&15.346&0.068\\\hline
\multirow{2}{*}{M12}&28.612&0.186&0.081&21.0&60.791&0.523&0.858&28.583&0.202&0.081\\&28.657&0.2&0.081&34.0&47.764&1.063&3.551&28.657&0.297&0.081\\\hline
\multirow{2}{*}{M13}&29.879&0.953&0.164&17.0&43.767&1.479&6.876&29.856&0.927&0.164\\&29.882&0.945&0.164&16.0&45.199&1.347&5.698&29.875&0.924&0.164\\\hline
\multirow{2}{*}{M14}&30.703&0.111&0.077&20.0&90.168&0.38&0.454&30.7&0.121&0.077\\&30.914&0.237&0.077&36.0&127.607&0.484&0.737&30.94&0.25&0.077\\\hline
\multirow{2}{*}{M15}&37.984&1.227&0.022&28.0&69.341&0.234&0.171&37.988&1.22&0.022\\&37.991&1.223&0.022&27.0&69.369&0.225&0.159&37.996&1.213&0.022\\\hline
\multirow{2}{*}{M16}&45.886&0.434&0.043&10.0&82.853&0.107&0.036&45.882&0.436&0.043\\&45.992&0.415&0.043&16.0&151.199&0.095&0.028&45.993&0.423&0.043\\\hline
\multirow{2}{*}{M17}&46.472&0.698&0.076&18.0&374.01&0.079&0.02&46.478&0.689&0.076\\&46.532&0.641&0.077&13.0&401.096&0.053&0.009&46.541&0.639&0.077\\\hline
\multirow{2}{*}{M18}&47.11&0.555&0.031&13.0&449.089&0.02&0.001&47.119&0.553&0.031\\&47.265&0.859&0.031&12.0&5053.62&0.002&0.0&47.264&0.859&0.031\\\hline
\multirow{2}{*}{M19}&47.295&0.58&0.108&12.0&614.777&0.042&0.006&47.289&0.579&0.108\\&47.318&0.406&0.108&12.0&189.89&0.136&0.058&47.31&0.407&0.108\\\hline
\multirow{2}{*}{M20}&47.958&0.15&0.037&19.0&263.285&0.055&0.01&47.944&0.153&0.037\\&48.038&0.031&0.038&15.0&486.718&0.024&0.002&48.046&0.035&0.038\\\hline
\multirow{2}{*}{M21}&117.091&18.851&0.048&47.0&46.232&0.895&2.514&117.093&18.876&0.048\\&117.332&19.137&0.048&22.0&23.659&0.816&2.092&117.293&19.067&0.048\\\hline
\multirow{2}{*}{M22}&118.718&45.715&0.053&12.0&101.171&0.147&0.068&118.721&45.71&0.053\\&119.197&45.838&0.053&29.0&82.042&0.439&0.605&119.19&45.822&0.053\\\hline
\multirow{2}{*}{M23}&125.384&23.173&0.093&16.0&26.297&0.671&1.416&125.357&23.146&0.093\\&125.392&23.191&0.093&15.0&29.454&0.565&1.002&125.376&23.154&0.093\\\hline
\multirow{2}{*}{M24*}&125.439&47.126&0.128&13.0&38.844&0.669&1.406&125.482&47.126&0.128\\&125.53&47.11&0.128&20.0&47.483&0.842&2.225&125.529&47.1&0.128\\\hline
\multirow{2}{*}{M25}&126.048&18.783&0.099&12.0&19.904&0.726&1.658&126.045&18.782&0.099\\&126.072&18.781&0.099&11.0&19.245&0.691&1.498&126.06&18.782&0.099\\\hline
\multirow{2}{*}{M26}&129.443&17.114&0.116&24.0&32.909&1.261&4.994&129.436&17.069&0.116\\&129.459&17.117&0.116&26.0&33.189&1.357&5.784&129.448&17.096&0.116\\\hline
\multirow{2}{*}{M27}&133.046&29.423&0.084&14.0&42.554&0.359&0.405&133.042&29.424&0.084\\&133.048&29.423&0.085&13.0&46.394&0.306&0.294&133.043&29.409&0.085\\\hline
\multirow{2}{*}{M28}&133.507&29.051&0.085&45.0&63.413&0.771&1.866&133.484&29.058&0.085\\&133.516&29.054&0.085&40.0&71.437&0.61&1.169&133.521&29.064&0.085\\\hline
\multirow{2}{*}{M29}&141.837&14.876&0.136&11.0&24.364&0.791&1.964&141.834&14.879&0.136\\&141.85&14.874&0.136&12.0&24.108&0.871&2.384&141.842&14.864&0.136\\\hline
\multirow{2}{*}{M30*}&146.422&34.666&0.134&42.0&56.753&1.761&9.746&146.36&34.722&0.134\\&146.523&34.629&0.134&25.0&99.155&0.609&1.164&146.526&34.626&0.134\\\hline
\multirow{2}{*}{M31*}&146.778&54.403&0.046&38.0&57.026&0.319&0.32&146.778&54.403&0.046\\&146.84&54.473&0.047&6.0&53.72&0.056&0.01&146.84&54.473&0.047\\\hline
\multirow{2}{*}{M32*}&152.33&54.239&0.046&16.0&62.774&0.193&0.117&152.348&54.234&0.046\\&152.514&54.515&0.046&11.0&50.205&0.165&0.085&152.519&54.511&0.046\\\hline
\multirow{2}{*}{M33*}&155.208&38.57&0.054&19.0&47.476&0.364&0.416&155.239&38.556&0.054\\&155.576&38.53&0.054&35.0&92.63&0.345&0.373&155.573&38.525&0.054\\\hline
\multirow{2}{*}{M34}&155.779&13.064&0.032&10.0&26.106&0.212&0.141&155.789&13.073&0.032\\&155.856&12.829&0.032&13.0&74.373&0.098&0.03&155.856&12.835&0.032\\\hline
\multirow{2}{*}{M35*}&157.519&41.131&0.091&22.0&85.509&0.333&0.348&157.532&41.125&0.091\\&157.585&41.144&0.091&31.0&61.573&0.649&1.323&157.612&41.16&0.091\\\hline
\multirow{2}{*}{M36*}&162.89&55.338&0.074&32.0&87.245&0.475&0.71&162.893&55.335&0.074\\&162.908&55.341&0.074&30.0&89.276&0.436&0.598&162.91&55.342&0.074\\\hline
\multirow{2}{*}{M37*}&167.984&57.082&0.047&22.0&75.114&0.263&0.217&167.954&57.086&0.047\\&168.51&56.989&0.047&15.0&33.264&0.401&0.505&168.532&57.002&0.047\\\hline
\multirow{2}{*}{M38*}&169.867&54.528&0.107&14.0&25.401&0.866&2.356&169.853&54.547&0.107\\&169.881&54.511&0.107&13.0&25.874&0.791&1.964&169.858&54.527&0.107\\\hline
\multirow{2}{*}{M39*}&170.265&34.409&0.035&11.0&26.917&0.274&0.235&170.264&34.373&0.035\\&170.56&34.345&0.035&34.0&71.248&0.32&0.322&170.589&34.313&0.035\\\hline
\multirow{2}{*}{M40}&170.969&20.49&0.107&10.0&30.034&0.491&0.757&170.969&20.489&0.107\\&170.981&20.503&0.107&12.0&24.556&0.714&1.603&171.014&20.502&0.107\\\hline
\multirow{2}{*}{M41}&171.175&17.302&0.144&29.0&32.386&1.952&11.971&171.104&17.297&0.144\\&171.224&17.311&0.144&33.0&30.58&2.338&17.168&171.154&17.352&0.144\\\hline
\multirow{2}{*}{M42}&171.581&19.244&0.103&13.0&19.616&0.935&2.747&171.63&19.252&0.103\\&171.621&19.204&0.103&26.0&21.353&1.679&8.856&171.694&19.241&0.103\\\hline
\multirow{2}{*}{M43*}&172.416&55.411&0.068&37.0&96.544&0.389&0.476&172.43&55.431&0.068\\&172.422&55.411&0.068&36.0&100.213&0.365&0.418&172.437&55.426&0.068\\\hline
\multirow{2}{*}{M44*}&173.052&53.524&0.047&14.0&45.128&0.274&0.236&173.06&53.511&0.047\\&173.088&53.523&0.047&16.0&47.564&0.297&0.278&173.094&53.51&0.047\\\hline
\multirow{2}{*}{M45*}&173.151&56.194&0.074&14.0&34.552&0.456&0.653&173.107&56.232&0.074\\&173.162&56.18&0.074&11.0&56.154&0.222&0.154&173.16&56.186&0.074\\\hline
\multirow{2}{*}{M46}&173.484&14.385&0.081&10.0&14.943&0.55&0.952&173.496&14.402&0.081\\&173.49&14.375&0.081&11.0&14.813&0.613&1.181&173.512&14.387&0.081\\\hline
\multirow{2}{*}{M47}&173.945&13.681&0.08&28.0&48.398&0.476&0.712&173.956&13.683&0.08\\&173.949&13.685&0.079&26.0&46.958&0.451&0.64&173.966&13.687&0.079\\\hline
\multirow{2}{*}{M48}&175.881&7.5&0.097&23.0&63.605&0.471&0.697&175.885&7.513&0.097\\&175.884&7.497&0.097&24.0&64.766&0.483&0.733&175.885&7.507&0.097\\\hline
\multirow{2}{*}{M49*}&176.018&33.448&0.032&21.0&51.768&0.256&0.206&176.015&33.434&0.032\\&176.455&33.277&0.032&45.0&52.484&0.539&0.914&176.429&33.336&0.032\\\hline
\multirow{2}{*}{M50}&176.038&5.776&0.104&31.0&70.166&0.532&0.89&176.047&5.766&0.104\\&176.039&5.776&0.104&34.0&71.841&0.57&1.021&176.049&5.769&0.104\\\hline
\multirow{2}{*}{M51}&176.106&7.671&0.066&22.0&34.348&0.608&1.162&176.088&7.634&0.066\\&176.109&7.689&0.066&20.0&34.499&0.551&0.955&176.093&7.656&0.066\\\hline
\multirow{2}{*}{M52*}&177.833&55.122&0.079&14.0&72.28&0.275&0.237&177.853&55.128&0.079\\&177.847&55.127&0.08&15.0&68.557&0.312&0.305&177.866&55.134&0.08\\\hline
\multirow{2}{*}{M53}&180.508&20.224&0.024&13.0&14.999&0.261&0.215&180.543&20.25&0.024\\&181.023&20.253&0.023&45.0&64.833&0.218&0.149&181.027&20.274&0.023\\\hline
\multirow{2}{*}{M54}&181.122&1.839&0.02&50.0&85.134&0.276&0.239&181.132&1.825&0.02\\&181.2&2.432&0.02&10.0&24.911&0.187&0.11&181.205&2.418&0.02\\\hline
\multirow{2}{*}{M55}&186.349&9.39&0.09&12.0&30.022&0.414&0.538&186.347&9.405&0.09\\&186.366&9.384&0.09&10.0&35.402&0.294&0.271&186.372&9.388&0.09\\\hline
\multirow{2}{*}{M56}&189.794&17.753&0.065&15.0&59.244&0.23&0.166&189.783&17.753&0.065\\&189.8&17.753&0.065&19.0&49.677&0.345&0.374&189.815&17.742&0.065\\\hline
\multirow{2}{*}{M57*}&197.143&43.751&0.036&10.0&38.336&0.177&0.098&197.149&43.75&0.036\\&197.179&43.447&0.036&31.0&35.714&0.577&1.044&197.162&43.508&0.036\\\hline
\multirow{2}{*}{M58*}&198.852&39.698&0.073&17.0&31.421&0.567&1.01&198.835&39.688&0.073\\&198.887&39.698&0.073&25.0&28.717&0.9&2.547&198.908&39.676&0.073\\\hline
\multirow{2}{*}{M59*}&200.438&57.523&0.118&21.0&70.012&0.635&1.268&200.485&57.54&0.118\\&200.465&57.526&0.118&20.0&69.472&0.61&1.169&200.496&57.544&0.118\\\hline
\multirow{2}{*}{M60}&201.568&0.21&0.082&23.0&65.376&0.313&0.307&201.581&0.196&0.082\\&201.579&0.215&0.082&19.0&66.818&0.253&0.202&201.589&0.213&0.082\\\hline
\multirow{2}{*}{M61}&201.745&1.224&0.083&22.0&57.814&0.34&0.362&201.745&1.226&0.083\\&201.752&1.223&0.083&18.0&58.673&0.274&0.236&201.768&1.222&0.083\\\hline
\multirow{2}{*}{M62}&206.297&26.894&0.075&11.0&40.884&0.247&0.191&206.294&26.901&0.075\\&206.298&26.897&0.075&10.0&40.796&0.225&0.159&206.304&26.902&0.075\\\hline
\multirow{2}{*}{M63}&207.092&25.677&0.052&38.0&103.235&0.464&0.678&207.073&25.686&0.052\\&207.097&25.675&0.052&31.0&122.058&0.321&0.323&207.107&25.673&0.052\\\hline
\multirow{2}{*}{M64}&213.495&1.91&0.053&14.0&27.436&0.347&0.378&213.528&1.893&0.053\\&213.632&1.738&0.054&11.0&53.322&0.142&0.063&213.63&1.732&0.054\\\hline
\multirow{2}{*}{M65*}&215.371&35.174&0.193&16.0&29.881&2.484&19.39&215.387&35.118&0.193\\&215.416&35.176&0.193&14.0&29.898&2.177&14.892&215.451&35.134&0.193\\\hline
\multirow{2}{*}{M66}&216.018&26.211&0.037&34.0&45.668&0.468&0.689&216.025&26.227&0.037\\&216.141&26.641&0.037&10.0&34.52&0.182&0.105&216.147&26.637&0.037\\\hline
\multirow{2}{*}{M67*}&216.298&38.71&0.166&11.0&70.052&0.465&0.679&216.308&38.716&0.166\\&216.301&38.715&0.167&12.0&57.269&0.622&1.215&216.309&38.735&0.167\\\hline
\multirow{2}{*}{M68}&217.859&24.687&0.097&16.0&36.607&0.581&1.059&217.862&24.689&0.097\\&217.877&24.694&0.097&14.0&35.194&0.529&0.878&217.883&24.694&0.097\\\hline
\multirow{2}{*}{M69}&218.614&26.325&0.095&10.0&36.666&0.364&0.416&218.611&26.318&0.095\\&218.616&26.334&0.095&11.0&33.869&0.432&0.587&218.628&26.322&0.095\\\hline
\multirow{2}{*}{M70}&218.647&24.712&0.08&12.0&15.804&0.835&2.188&218.618&24.709&0.08\\&218.714&24.713&0.08&11.0&16.68&0.732&1.685&218.642&24.722&0.08\\\hline
\multirow{2}{*}{M71}&222.941&22.566&0.117&30.0&46.35&0.932&2.731&222.921&22.561&0.117\\&222.959&22.552&0.117&22.0&40.827&0.774&1.884&222.956&22.545&0.117\\\hline
\multirow{2}{*}{M72}&223.592&21.629&0.1&18.0&44.638&0.546&0.937&223.607&21.638&0.1\\&223.601&21.632&0.1&17.0&45.988&0.501&0.789&223.613&21.649&0.1\\\hline
\multirow{2}{*}{M73}&223.673&22.663&0.105&12.0&24.182&0.676&1.437&223.689&22.648&0.105\\&223.675&22.694&0.105&10.0&26.216&0.523&0.859&223.697&22.682&0.105\\\hline
\multirow{2}{*}{M74}&223.927&19.28&0.059&13.0&21.573&0.462&0.669&223.955&19.241&0.059\\&223.963&19.281&0.059&15.0&24.859&0.464&0.676&223.96&19.26&0.059\\\hline
\multirow{2}{*}{M75*}&226.253&47.498&0.088&12.0&33.272&0.903&2.562&226.283&47.489&0.088\\&226.47&47.422&0.088&20.0&31.052&1.603&8.071&226.455&47.324&0.088\\\hline
\multirow{2}{*}{M76*}&227.488&33.462&0.112&48.0&72.038&0.635&1.269&227.488&33.462&0.112\\&227.57&33.495&0.112&10.0&71.98&0.13&0.053&227.57&33.495&0.112\\\hline
\multirow{2}{*}{M77}&230.387&29.321&0.113&32.0&41.01&1.238&4.819&230.39&29.303&0.113\\&230.393&29.275&0.113&39.0&47.492&1.299&5.301&230.4&29.268&0.113\\\hline
\multirow{2}{*}{M78}&230.754&20.467&0.04&10.0&22.608&0.278&0.243&230.733&20.489&0.04\\&231.089&20.757&0.04&32.0&64.444&0.316&0.314&231.089&20.757&0.04\\\hline
\multirow{2}{*}{M79*}&230.808&30.886&0.074&18.0&36.501&0.484&0.737&230.817&30.91&0.074\\&230.848&31.056&0.074&35.0&40.454&0.845&2.242&230.902&31.02&0.074\\\hline
\multirow{2}{*}{M80}&230.843&28.613&0.083&13.0&31.139&0.383&0.461&230.86&28.601&0.083\\&230.853&28.615&0.083&14.0&31.693&0.405&0.515&230.862&28.61&0.083\\\hline
\multirow{2}{*}{M81}&231.484&29.83&0.114&24.0&54.781&0.695&1.515&231.493&29.815&0.114\\&231.637&29.688&0.114&47.0&43.49&1.686&8.93&231.679&29.709&0.114\\\hline
\multirow{2}{*}{M82}&232.451&29.015&0.085&18.0&41.086&0.415&0.542&232.465&29.01&0.085\\&232.468&29.027&0.085&16.0&41.971&0.362&0.411&232.468&29.025&0.085\\\hline
\multirow{2}{*}{M83}&233.657&25.22&0.034&11.0&39.019&0.17&0.091&233.677&25.22&0.034\\&233.987&25.216&0.035&14.0&25.09&0.332&0.347&234.001&25.262&0.035\\\hline
\multirow{2}{*}{M84}&234.895&21.789&0.042&72.0&113.271&0.42&0.554&234.893&21.787&0.042\\&235.18&21.416&0.042&15.0&30.615&0.319&0.319&235.185&21.42&0.042\\\hline
\multirow{2}{*}{M85*}&236.785&35.63&0.079&10.0&35.561&0.328&0.339&236.787&35.609&0.079\\&236.788&35.614&0.079&11.0&31.406&0.407&0.519&236.805&35.597&0.079\\\hline
\multirow{2}{*}{M86}&238.848&28.993&0.078&23.0&51.188&0.398&0.499&238.859&29.012&0.078\\&238.898&28.85&0.077&11.0&26.625&0.364&0.416&238.922&28.84&0.077\\\hline
\multirow{2}{*}{M87}&240.758&16.249&0.037&30.0&45.467&0.298&0.279&240.757&16.248&0.037\\&241.099&17.076&0.036&636.0&108.56&2.5&19.63&241.047&17.025&0.036\\\hline
\multirow{2}{*}{M88}&240.869&17.188&0.034&12.0&40.839&0.126&0.05&240.849&17.191&0.034\\&241.338&17.76&0.034&45.0&108.32&0.178&0.1&241.331&17.762&0.034\\\hline
\multirow{2}{*}{M89}&241.428&16.339&0.044&34.0&58.727&0.394&0.489&241.436&16.326&0.044\\&241.433&16.338&0.044&37.0&58.697&0.43&0.58&241.449&16.314&0.044\\\hline
\multirow{2}{*}{M90}&241.976&25.493&0.041&11.0&33.777&0.187&0.11&241.973&25.489&0.041\\&242.421&25.687&0.041&11.0&27.117&0.231&0.168&242.416&25.699&0.041\\\hline
\multirow{2}{*}{M91}&243.034&29.529&0.032&14.0&14.063&0.418&0.549&243.063&29.513&0.032\\&243.181&29.469&0.032&11.0&42.533&0.114&0.041&243.179&29.459&0.032\\\hline
\multirow{3}{*}{M92*}&246.28&40.867&0.029&15.0&36.042&0.191&0.114&246.324&40.861&0.029\\&246.681&40.916&0.029&10.0&29.234&0.156&0.077&246.682&40.955&0.029\\&247.546&40.722&0.029&49.0&69.835&0.32&0.323&247.537&40.739&0.029\\\hline
\multirow{2}{*}{M93*}&247.084&40.896&0.032&17.0&42.541&0.177&0.099&247.109&40.884&0.032\\&247.301&40.611&0.031&12.0&38.055&0.14&0.062&247.307&40.608&0.031\\\hline
\multirow{2}{*}{M94*}&247.827&39.795&0.03&16.0&39.155&0.185&0.108&247.82&39.83&0.03\\&247.83&39.797&0.03&17.0&38.727&0.199&0.125&247.824&39.839&0.03\\\hline
\multirow{2}{*}{M95}&257.739&63.708&0.081&21.0&41.516&0.55&0.951&257.759&63.731&0.081\\&258.204&64.056&0.081&178.0&273.981&0.716&1.609&258.187&64.054&0.081\\\hline
\multirow{2}{*}{M96*}&258.928&64.637&0.08&18.0&35.81&0.544&0.93&258.92&64.649&0.08\\&258.974&64.663&0.08&21.0&36.678&0.619&1.203&258.967&64.667&0.08\\\hline
\multirow{2}{*}{M97*}&260.564&30.752&0.046&31.0&185.115&0.347&0.379&260.574&30.756&0.046\\&260.963&30.813&0.046&12.0&99.034&0.247&0.191&260.949&30.818&0.046\\\hline
\multirow{2}{*}{M98}&312.975&1.049&0.147&24.0&108.011&1.144&4.109&312.989&1.029&0.147\\&312.988&1.07&0.146&23.0&107.259&1.097&3.781&312.992&1.039&0.146\\\hline
\multirow{3}{*}{M99}&333.15&13.968&0.027&25.0&75.547&0.276&0.239&333.152&13.983&0.027\\&333.923&13.742&0.026&12.0&62.527&0.158&0.079&333.92&13.743&0.026\\&333.926&13.77&0.026&18.0&67.04&0.222&0.155&333.944&13.767&0.026\\\hline


==> tables/ppm.tex <==
\multirow{2}{*}{PPM1}&0.465&1.041&0.086&16.0&46.377&0.534&0.894&0.459&1.054&0.086\\&0.989&0.546&0.085&28.0&42.974&0.986&3.057&0.885&0.578&0.085\\\hline
\multirow{2}{*}{PPM2}&0.597&0.535&0.08&19.0&50.209&0.573&1.033&0.616&0.553&0.08\\&0.808&1.07&0.079&30.0&54.784&0.828&2.156&0.786&1.054&0.079\\\hline
\multirow{2}{*}{PPM3}&1.259&0.992&0.1&44.0&65.095&1.26&4.991&1.25&0.998&0.1\\&1.869&0.876&0.101&13.0&37.76&0.64&1.288&1.863&0.869&0.101\\\hline
\multirow{2}{*}{PPM4}&1.496&0.505&0.062&17.0&37.769&0.617&1.197&1.514&0.555&0.062\\&2.477&0.38&0.062&10.0&32.179&0.429&0.577&2.47&0.387&0.062\\\hline
\multirow{2}{*}{PPM5}&1.916&14.775&0.117&12.0&74.476&0.372&0.435&1.912&14.784&0.117\\&1.927&14.476&0.117&11.0&36.054&0.685&1.472&1.935&14.455&0.117\\\hline
\multirow{2}{*}{PPM6}&2.799&0.741&0.111&10.0&20.414&0.926&2.692&2.775&0.716&0.111\\&3.024&0.387&0.111&15.0&30.449&0.942&2.786&3.009&0.374&0.111\\\hline
\multirow{2}{*}{PPM7}&3.2&0.127&0.063&16.0&30.195&0.712&1.593&3.222&0.155&0.063\\&3.719&0.694&0.063&15.0&43.609&0.466&0.682&3.713&0.721&0.063\\\hline
\multirow{2}{*}{PPM8}&4.797&0.343&0.144&13.0&32.312&1.129&4.002&4.792&0.33&0.144\\&5.275&0.637&0.144&18.0&35.388&1.422&6.353&5.287&0.69&0.144\\\hline
\multirow{2}{*}{PPM9}&10.257&14.488&0.197&21.0&53.162&1.299&5.305&10.305&14.502&0.197\\&10.373&14.008&0.197&18.0&30.106&1.918&11.562&10.446&13.988&0.197\\\hline
\multirow{2}{*}{PPM10*}&10.26&15.402&0.084&12.0&88.319&0.352&0.39&10.276&15.386&0.084\\&10.305&15.378&0.083&10.0&91.975&0.279&0.245&10.305&15.378&0.083\\\hline
\multirow{3}{*}{PPM11*}&11.448&15.422&0.078&22.0&142.294&0.348&0.381&11.458&15.449&0.078\\&11.774&15.512&0.079&42.0&151.091&0.634&1.262&11.812&15.464&0.079\\&12.684&15.926&0.078&20.0&108.961&0.415&0.542&12.683&15.923&0.078\\\hline
\multirow{2}{*}{PPM12}&13.242&6.007&0.151&38.0&73.17&1.505&7.118&13.27&6.061&0.151\\&13.764&5.778&0.151&22.0&120.98&0.53&0.882&13.756&5.767&0.151\\\hline
\multirow{3}{*}{PPM13}&13.517&0.994&0.043&26.0&59.225&0.484&0.735&13.594&0.995&0.043\\&13.564&0.994&0.043&27.0&57.23&0.519&0.846&13.603&1.003&0.043\\&14.03&0.196&0.044&45.0&101.904&0.493&0.765&14.036&0.2&0.044\\\hline
\multirow{2}{*}{PPM14}&15.249&0.563&0.11&13.0&33.539&1.017&3.249&15.271&0.544&0.11\\&15.614&0.112&0.111&11.0&18.783&1.506&7.129&15.587&0.117&0.111\\\hline
\multirow{6}{*}{PPM15*}&17.518&15.799&0.061&10.0&64.918&0.289&0.263&17.509&15.776&0.061\\&17.519&15.758&0.06&12.0&61.098&0.369&0.428&17.525&15.745&0.06\\&17.567&15.07&0.06&10.0&77.214&0.244&0.187&17.563&15.072&0.06\\&18.036&15.729&0.061&26.0&97.039&0.502&0.793&18.01&15.693&0.061\\&18.075&15.739&0.061&19.0&132.174&0.27&0.229&18.06&15.747&0.061\\&18.589&15.247&0.061&11.0&54.528&0.376&0.445&18.572&15.236&0.061\\\hline
\multirow{4}{*}{PPM16}&17.574&0.421&0.045&37.0&41.77&0.802&2.019&17.633&0.483&0.045\\&17.779&0.575&0.046&21.0&29.845&0.637&1.274&17.754&0.593&0.046\\&19.149&0.581&0.045&11.0&24.945&0.401&0.504&19.121&0.622&0.045\\&19.763&0.419&0.045&14.0&21.315&0.589&1.092&19.742&0.442&0.045\\\hline
\multirow{2}{*}{PPM17}&18.496&14.378&0.059&27.0&36.915&0.967&2.94&18.425&14.362&0.059\\&18.764&13.525&0.059&25.0&50.227&0.679&1.449&18.75&13.558&0.059\\\hline
\multirow{2}{*}{PPM18}&20.028&14.863&0.054&18.0&41.917&0.478&0.718&20.068&14.842&0.054\\&20.561&14.285&0.053&11.0&20.298&0.574&1.037&20.588&14.294&0.053\\\hline
\multirow{2}{*}{PPM19}&22.428&0.676&0.118&12.0&18.455&1.496&7.035&22.399&0.649&0.118\\&22.845&0.694&0.118&11.0&86.392&0.298&0.279&22.865&0.698&0.118\\\hline
\multirow{2}{*}{PPM20*}&23.671&16.175&0.071&20.0&98.658&0.377&0.446&23.655&16.184&0.071\\&23.854&15.317&0.071&32.0&131.104&0.455&0.65&23.855&15.325&0.071\\\hline
\multirow{2}{*}{PPM21}&27.022&14.332&0.07&10.0&18.337&0.749&1.763&27.008&14.377&0.07\\&27.309&13.993&0.07&37.0&104.797&0.495&0.771&27.313&13.988&0.07\\\hline
\multirow{2}{*}{PPM22}&27.067&12.929&0.158&48.0&85.306&1.813&10.326&27.115&13.014&0.158\\&27.448&13.689&0.158&25.0&55.76&1.447&6.574&27.505&13.687&0.158\\\hline
\multirow{2}{*}{PPM23}&30.703&0.111&0.077&20.0&90.168&0.38&0.454&30.7&0.121&0.077\\&31.297&0.175&0.077&15.0&81.345&0.311&0.303&31.298&0.189&0.077\\\hline
\multirow{2}{*}{PPM24}&30.815&0.311&0.042&10.0&368.24&0.032&0.003&30.814&0.31&0.042\\&31.617&0.72&0.042&44.0&103.212&0.5&0.785&31.635&0.754&0.042\\\hline
\multirow{2}{*}{PPM25}&31.05&0.411&0.172&39.0&78.256&1.929&11.686&30.988&0.419&0.172\\&31.466&0.094&0.173&34.0&114.112&1.157&4.204&31.45&0.11&0.173\\\hline
\multirow{2}{*}{PPM26}&32.243&12.397&0.061&16.0&66.09&0.495&0.771&32.236&12.419&0.061\\&32.893&13.01&0.061&16.0&63.843&0.516&0.835&32.902&12.999&0.061\\\hline
\multirow{2}{*}{PPM27}&35.187&0.83&0.128&24.0&106.703&0.581&1.061&35.164&0.786&0.128\\&35.718&0.879&0.129&42.0&105.159&1.006&3.178&35.708&0.873&0.129\\\hline
\multirow{2}{*}{PPM28}&35.684&0.13&0.041&20.0&1296035.903&0.0&0.0&35.684&0.13&0.041\\&37.087&0.685&0.041&19.0&476.181&0.048&0.007&37.083&0.673&0.041\\\hline
\multirow{2}{*}{PPM29}&37.234&0.371&0.021&12.0&2431.303&0.003&0.0&37.232&0.371&0.021\\&38.162&0.645&0.021&50.0&154.773&0.189&0.112&38.142&0.719&0.021\\\hline
\multirow{2}{*}{PPM30}&41.293&1.235&0.076&30.0&115.575&0.42&0.554&41.305&1.238&0.076\\&41.693&0.56&0.076&11.0&34.151&0.526&0.868&41.66&0.561&0.076\\\hline
\multirow{2}{*}{PPM31}&43.155&0.405&0.17&23.0&57.18&1.571&7.75&43.206&0.426&0.17\\&43.97&0.415&0.17&23.0&45.612&1.963&12.107&44.015&0.387&0.17\\\hline
\multirow{2}{*}{PPM32}&45.886&0.434&0.043&10.0&82.853&0.107&0.036&45.882&0.436&0.043\\&46.288&0.346&0.043&21.0&630.445&0.03&0.003&46.293&0.353&0.043\\\hline
\multirow{5}{*}{PPM33}&46.399&0.625&0.075&14.0&527.799&0.044&0.006&46.396&0.63&0.075\\&46.472&0.698&0.076&18.0&374.01&0.079&0.02&46.478&0.689&0.076\\&46.532&0.641&0.077&13.0&401.096&0.053&0.009&46.541&0.639&0.077\\&46.627&0.12&0.077&11.0&1347.655&0.013&0.001&46.626&0.122&0.077\\&46.719&0.138&0.076&22.0&448.453&0.081&0.021&46.73&0.137&0.076\\\hline
\multirow{2}{*}{PPM34}&47.078&0.787&0.156&10.0&54464.148&0.001&0.0&47.078&0.787&0.156\\&47.186&1.005&0.156&13.0&3356.634&0.013&0.001&47.185&1.005&0.156\\\hline
\multirow{2}{*}{PPM35}&47.149&0.641&0.107&13.0&603.188&0.044&0.006&47.153&0.645&0.107\\&47.512&0.718&0.106&11.0&518.586&0.044&0.006&47.516&0.722&0.106\\\hline
\multirow{2}{*}{PPM36}&47.334&0.733&0.083&11.0&496.517&0.038&0.004&47.338&0.731&0.083\\&47.557&0.952&0.083&11.0&443.176&0.042&0.005&47.55&0.951&0.083\\\hline
\multirow{2}{*}{PPM37}&47.489&0.698&0.13&10.0&88.807&0.234&0.172&47.502&0.677&0.13\\&47.738&0.356&0.129&17.0&238.977&0.151&0.071&47.752&0.366&0.129\\\hline
\multirow{4}{*}{PPM38}&47.617&1.098&0.038&12.0&4138.687&0.002&0.0&47.618&1.098&0.038\\&47.958&0.15&0.037&19.0&263.285&0.055&0.01&47.944&0.153&0.037\\&48.038&0.031&0.038&15.0&486.718&0.024&0.002&48.046&0.035&0.038\\&48.121&0.124&0.038&11.0&574.719&0.015&0.001&48.126&0.122&0.038\\\hline
\multirow{2}{*}{PPM39}&48.462&0.325&0.131&11.0&871.812&0.025&0.002&48.46&0.327&0.131\\&48.76&0.134&0.131&17.0&154.317&0.221&0.154&48.762&0.136&0.131\\\hline
\multirow{2}{*}{PPM40}&48.462&1.098&0.071&12.0&304.178&0.067&0.014&48.467&1.11&0.071\\&48.546&1.102&0.07&13.0&519.234&0.042&0.006&48.541&1.109&0.07\\\hline
\multirow{2}{*}{PPM41}&112.08&41.5&0.118&37.0&61.261&1.421&6.342&112.035&41.48&0.118\\&112.668&40.883&0.119&36.0&112.156&0.767&1.848&112.632&40.901&0.119\\\hline
\multirow{2}{*}{PPM42}&116.422&33.946&0.063&44.0&87.049&0.709&1.581&116.452&33.947&0.063\\&117.625&33.791&0.062&10.0&38.524&0.367&0.424&117.667&33.811&0.062\\\hline
\multirow{2}{*}{PPM43}&118.317&38.874&0.041&12.0&33.326&0.462&0.67&118.333&38.85&0.041\\&119.652&37.771&0.041&50.0&97.878&0.674&1.428&119.591&37.705&0.041\\\hline
\multirow{2}{*}{PPM44}&118.351&34.276&0.14&50.0&179.629&0.783&1.928&118.325&34.278&0.14\\&118.819&34.455&0.14&16.0&34.641&1.311&5.403&118.894&34.452&0.14\\\hline
\multirow{2}{*}{PPM45}&118.976&33.784&0.075&23.0&48.304&0.621&1.211&118.974&33.798&0.075\\&118.982&34.134&0.074&12.0&68.397&0.229&0.165&118.98&34.132&0.074\\\hline
\multirow{2}{*}{PPM46}&118.996&41.179&0.074&22.0&72.192&0.399&0.499&118.946&41.198&0.074\\&119.481&40.873&0.074&12.0&28.621&0.542&0.923&119.454&40.877&0.074\\\hline
\multirow{2}{*}{PPM47}&119.137&30.679&0.158&18.0&31.396&2.243&15.803&119.107&30.662&0.158\\&119.182&31.352&0.157&17.0&46.918&1.383&6.009&119.133&31.314&0.157\\\hline
\multirow{2}{*}{PPM48}&120.327&27.227&0.047&11.0&26.244&0.375&0.442&120.327&27.283&0.047\\&120.957&26.513&0.048&14.0&44.158&0.29&0.265&120.928&26.511&0.048\\\hline
\multirow{2}{*}{PPM49*}&120.848&39.932&0.041&14.0&38.731&0.353&0.391&120.919&39.935&0.041\\&122.148&38.914&0.041&35.0&89.704&0.382&0.459&122.116&38.914&0.041\\\hline
\multirow{2}{*}{PPM50}&120.966&10.029&0.034&27.0&69.311&0.4&0.503&120.982&10.037&0.034\\&121.214&10.562&0.034&14.0&27.325&0.525&0.867&121.261&10.572&0.034\\\hline
\multirow{2}{*}{PPM51*}&122.354&48.96&0.116&16.0&66.297&0.43&0.581&122.356&48.965&0.116\\&122.707&49.199&0.117&35.0&116.849&0.534&0.896&122.726&49.207&0.117\\\hline
\multirow{2}{*}{PPM52}&124.718&22.956&0.094&40.0&37.298&1.194&4.479&124.752&22.994&0.094\\&124.97&23.456&0.095&33.0&41.548&0.906&2.58&124.993&23.457&0.095\\\hline
\multirow{2}{*}{PPM53*}&124.883&54.6&0.081&10.0&72.818&0.215&0.145&124.863&54.595&0.081\\&125.378&55.02&0.081&45.0&131.956&0.532&0.89&125.376&55.042&0.081\\\hline
\multirow{3}{*}{PPM54*}&125.439&47.126&0.128&13.0&38.844&0.669&1.406&125.482&47.126&0.128\\&125.53&47.11&0.128&27.0&47.483&0.842&2.225&125.529&47.1&0.128\\&126.371&47.156&0.127&50.0&119.104&0.96&2.898&126.376&47.154&0.127\\\hline
\multirow{2}{*}{PPM55}&125.636&6.915&0.082&17.0&51.607&0.469&0.692&125.658&6.922&0.082\\&126.096&7.409&0.082&10.0&30.057&0.47&0.695&126.096&7.422&0.082\\\hline
\multirow{2}{*}{PPM56}&125.755&16.024&0.152&50.0&60.422&2.68&22.566&125.699&16.044&0.152\\&126.459&15.865&0.153&14.0&23.961&1.578&7.825&126.478&15.893&0.153\\\hline
\multirow{2}{*}{PPM57*}&125.778&44.125&0.148&16.0&43.946&0.817&2.096&125.76&44.123&0.148\\&125.819&44.347&0.147&10.0&41.736&0.535&0.9&125.851&44.334&0.147\\\hline
\multirow{2}{*}{PPM58}&126.632&17.469&0.089&35.0&53.209&0.713&1.598&126.637&17.463&0.089\\&127.27&17.891&0.089&16.0&24.049&0.712&1.591&127.253&17.83&0.089\\\hline
\multirow{2}{*}{PPM59}&126.714&18.17&0.101&19.0&46.444&0.524&0.862&126.709&18.181&0.101\\&127.213&17.598&0.101&33.0&25.569&1.599&8.029&127.157&17.554&0.101\\\hline
\multirow{3}{*}{PPM60*}&126.717&53.946&0.031&14.0&38.592&0.271&0.23&126.646&53.967&0.031\\&127.016&54.821&0.031&19.0&43.238&0.326&0.335&127.059&54.796&0.031\\&128.276&54.554&0.031&10.0&34.613&0.215&0.146&128.228&54.564&0.031\\\hline
\multirow{2}{*}{PPM61*}&126.726&42.274&0.116&14.0&30.96&0.886&2.468&126.693&42.305&0.116\\&126.958&42.759&0.116&16.0&113.565&0.279&0.245&126.967&42.754&0.116\\\hline
\multirow{2}{*}{PPM62*}&128.979&49.059&0.175&10.0&21.532&1.653&8.579&128.929&49.019&0.175\\&129.614&49.182&0.175&11.0&71.647&0.557&0.973&129.616&49.173&0.175\\\hline
\multirow{2}{*}{PPM63*}&130.709&36.119&0.054&24.0&52.23&0.4&0.502&130.704&36.134&0.054\\&131.873&35.488&0.054&15.0&31.909&0.407&0.519&131.906&35.52&0.054\\\hline
\multirow{4}{*}{PPM64}&133.046&29.423&0.084&14.0&42.554&0.359&0.405&133.042&29.424&0.084\\&133.048&29.423&0.085&13.0&46.394&0.306&0.294&133.043&29.409&0.085\\&133.507&29.051&0.085&45.0&63.413&0.771&1.866&133.484&29.058&0.085\\&133.516&29.054&0.085&40.0&71.437&0.61&1.169&133.521&29.064&0.085\\\hline
\multirow{2}{*}{PPM65}&133.15&16.321&0.099&18.0&41.281&0.543&0.927&133.179&16.323&0.099\\&133.19&15.725&0.1&16.0&32.692&0.615&1.187&133.219&15.739&0.1\\\hline
\multirow{2}{*}{PPM66}&135.067&14.706&0.102&19.0&45.755&0.649&1.324&135.088&14.708&0.102\\&135.613&14.395&0.101&12.0&40.5&0.458&0.658&135.595&14.404&0.101\\\hline
\multirow{3}{*}{PPM67}&135.933&20.354&0.082&12.0&38.708&0.336&0.355&135.924&20.353&0.082\\&136.136&19.948&0.084&28.0&64.213&0.487&0.744&136.14&19.942&0.084\\&136.491&19.211&0.083&11.0&38.906&0.313&0.307&136.49&19.228&0.083\\\hline
\multirow{3}{*}{PPM68*}&136.072&52.013&0.062&17.0&63.529&0.42&0.555&136.109&52.033&0.062\\&136.338&52.37&0.062&10.0&84.629&0.186&0.109&136.331&52.374&0.062\\&136.921&52.1&0.061&47.0&111.586&0.661&1.374&136.967&52.104&0.061\\\hline
\multirow{3}{*}{PPM69}&136.138&17.441&0.029&15.0&38.051&0.207&0.135&136.131&17.423&0.029\\&137.32&19.469&0.028&25.0&38.221&0.335&0.353&137.32&19.484&0.028\\&139.053&17.631&0.029&43.0&71.548&0.317&0.315&139.083&17.669&0.029\\\hline
\multirow{2}{*}{PPM70}&136.84&16.652&0.073&21.0&69.357&0.339&0.36&136.863&16.645&0.073\\&137.115&16.02&0.072&38.0&72.374&0.592&1.101&137.097&16.021&0.072\\\hline
\multirow{2}{*}{PPM71}&138.127&15.997&0.089&19.0&26.626&0.965&2.925&138.125&15.89&0.089\\&138.719&15.717&0.089&11.0&22.552&0.656&1.352&138.673&15.719&0.089\\\hline
\multirow{2}{*}{PPM72}&141.168&3.369&0.087&13.0&35.9&0.437&0.6&141.169&3.364&0.087\\&141.66&3.456&0.088&16.0&35.292&0.547&0.941&141.666&3.435&0.088\\\hline
\multirow{2}{*}{PPM73}&142.463&23.008&0.166&11.0&24.682&1.524&7.298&142.471&23.078&0.166\\&142.7&22.529&0.165&12.0&24.513&1.652&8.572&142.696&22.548&0.165\\\hline
\multirow{2}{*}{PPM74*}&143.881&54.614&0.046&12.0&38.585&0.252&0.2&143.907&54.631&0.046\\&146.417&54.646&0.046&27.0&84.067&0.265&0.22&146.419&54.658&0.046\\\hline
\multirow{2}{*}{PPM75}&143.908&12.303&0.18&13.0&27.7&1.569&7.732&143.854&12.314&0.18\\&144.342&12.741&0.18&18.0&26.555&2.254&15.963&144.382&12.75&0.18\\\hline
\multirow{2}{*}{PPM76*}&145.928&56.885&0.139&12.0&33.351&1.027&3.31&145.843&56.873&0.139\\&146.333&56.553&0.14&41.0&118.276&1.008&3.191&146.271&56.574&0.14\\\hline
\multirow{2}{*}{PPM77*}&146.12&34.816&0.133&17.0&32.944&1.205&4.561&146.115&34.864&0.133\\&146.422&34.666&0.134&42.0&56.753&1.761&9.746&146.36&34.722&0.134\\\hline
\multirow{2}{*}{PPM78}&146.586&43.147&0.073&93.0&91.761&1.297&5.287&146.592&43.173&0.073\\&146.863&42.153&0.073&10.0&28.485&0.45&0.636&146.899&42.142&0.073\\\hline
\multirow{2}{*}{PPM79}&146.769&23.238&0.084&15.0&39.96&0.419&0.551&146.786&23.22&0.084\\&147.375&22.676&0.084&15.0&21.624&0.752&1.777&147.371&22.671&0.084\\\hline
\multirow{2}{*}{PPM80}&146.878&0.687&0.063&12.0&32.434&0.41&0.529&146.896&0.647&0.063\\&147.165&0.434&0.063&13.0&67.126&0.218&0.149&147.142&0.454&0.063\\\hline
\multirow{3}{*}{PPM81}&147.2&6.141&0.091&16.0&32.887&0.597&1.121&147.225&6.143&0.091\\&147.449&5.782&0.091&16.0&33.093&0.592&1.102&147.436&5.79&0.091\\&147.773&6.215&0.091&15.0&16.284&1.091&3.739&147.812&6.24&0.091\\\hline
\multirow{2}{*}{PPM82}&148.087&0.985&0.047&12.0&43.76&0.29&0.264&148.101&0.994&0.047\\&148.73&0.757&0.047&15.0&16.877&0.9&2.545&148.708&0.683&0.047\\\hline
\multirow{2}{*}{PPM83}&148.389&1.698&0.099&36.0&37.911&1.318&5.454&148.391&1.684&0.099\\&148.922&1.602&0.1&17.0&50.913&0.488&0.748&148.928&1.621&0.1\\\hline
\multirow{2}{*}{PPM84*}&150.717&54.818&0.048&18.0&66.849&0.223&0.156&150.706&54.818&0.048\\&151.112&54.58&0.047&15.0&49.64&0.241&0.183&151.131&54.593&0.047\\\hline
\multirow{2}{*}{PPM85}&151.211&10.681&0.16&17.0&32.262&1.431&6.437&151.18&10.651&0.16\\&151.384&11.179&0.159&21.0&30.359&1.847&10.713&151.404&11.174&0.159\\\hline
\multirow{2}{*}{PPM86*}&151.257&53.125&0.045&23.0&101.845&0.169&0.089&151.271&53.115&0.045\\&152.33&54.239&0.046&16.0&62.774&0.193&0.117&152.348&54.234&0.046\\\hline
\multirow{2}{*}{PPM87}&152.755&8.699&0.097&11.0&25.541&0.494&0.768&152.748&8.699&0.097\\&153.094&8.695&0.097&15.0&28.546&0.602&1.14&153.097&8.698&0.097\\\hline
\multirow{2}{*}{PPM88}&152.972&3.289&0.046&22.0&93.613&0.174&0.095&152.964&3.295&0.046\\&154.229&3.822&0.046&14.0&196.394&0.053&0.009&154.229&3.821&0.046\\\hline
\multirow{2}{*}{PPM89}&154.258&3.854&0.106&11.0&43.428&0.333&0.348&154.271&3.831&0.106\\&154.508&3.339&0.105&23.0&104.522&0.286&0.257&154.498&3.334&0.105\\\hline
\multirow{2}{*}{PPM90}&155.217&25.54&0.021&14.0&34.31&0.208&0.136&155.22&25.547&0.021\\&156.241&28.029&0.021&11.0&42.632&0.133&0.055&156.201&28.031&0.021\\\hline
\multirow{2}{*}{PPM91}&155.269&21.676&0.041&12.0&29.846&0.278&0.243&155.277&21.668&0.041\\&156.658&21.681&0.042&12.0&30.713&0.27&0.229&156.643&21.692&0.042\\\hline
\multirow{2}{*}{PPM92}&156.003&1.494&0.097&12.0&40.399&0.344&0.372&156.002&1.491&0.097\\&156.449&1.19&0.097&15.0&64.335&0.271&0.231&156.46&1.2&0.097\\\hline
\multirow{2}{*}{PPM93*}&156.233&50.198&0.156&45.0&171.162&0.842&2.226&156.216&50.194&0.156\\&156.31&49.85&0.156&13.0&52.664&0.787&1.944&156.38&49.868&0.156\\\hline
\multirow{2}{*}{PPM94}&157.257&40.301&0.067&17.0&38.87&0.586&1.077&157.337&40.302&0.067\\&158.052&40.162&0.067&68.0&174.058&0.528&0.875&158.026&40.161&0.067\\\hline
\multirow{2}{*}{PPM95}&159.742&4.644&0.069&26.0&52.822&0.436&0.598&159.742&4.669&0.069\\&159.822&5.186&0.068&54.0&105.951&0.453&0.644&159.827&5.196&0.068\\\hline
\multirow{2}{*}{PPM96}&160.343&25.532&0.054&11.0&22.763&0.39&0.478&160.339&25.533&0.054\\&160.86&24.867&0.053&13.0&37.8&0.278&0.242&160.869&24.861&0.053\\\hline
\multirow{2}{*}{PPM97}&162.121&23.204&0.061&12.0&33.087&0.385&0.465&162.128&23.211&0.061\\&162.746&23.501&0.06&19.0&44.94&0.443&0.616&162.707&23.48&0.06\\\hline
\multirow{2}{*}{PPM98}&163.037&16.352&0.085&10.0&33.372&0.403&0.51&163.056&16.363&0.085\\&163.492&16.855&0.084&19.0&68.214&0.373&0.436&163.503&16.846&0.084\\\hline
\multirow{2}{*}{PPM99}&163.483&26.909&0.021&10.0&37.473&0.137&0.059&163.461&26.91&0.021\\&164.584&24.194&0.021&12.0&31.834&0.193&0.117&164.547&24.209&0.021\\\hline
\multirow{2}{*}{PPM100*}&163.494&54.846&0.072&32.0&84.633&0.466&0.683&163.475&54.862&0.072\\&163.789&54.789&0.071&16.0&58.273&0.334&0.35&163.783&54.793&0.071\\\hline
\multirow{2}{*}{PPM101}&164.557&29.628&0.053&11.0&35.911&0.249&0.196&164.549&29.625&0.053\\&164.9&29.869&0.054&13.0&51.591&0.212&0.141&164.888&29.87&0.054\\\hline
\multirow{2}{*}{PPM102*}&166.125&35.23&0.074&11.0&48.943&0.201&0.127&166.119&35.232&0.074\\&166.728&35.572&0.074&10.0&35.436&0.252&0.199&166.723&35.572&0.074\\\hline
\multirow{5}{*}{PPM103*}&167.338&41.557&0.076&22.0&77.288&0.266&0.222&167.337&41.544&0.076\\&167.85&39.602&0.076&15.0&38.768&0.357&0.399&167.876&39.612&0.076\\&167.93&40.855&0.075&41.0&104.533&0.359&0.404&167.927&40.849&0.075\\&168.021&40.534&0.075&31.0&64.65&0.431&0.584&168.037&40.526&0.075\\&168.393&40.285&0.075&43.0&86.323&0.453&0.645&168.403&40.273&0.075\\\hline
\multirow{2}{*}{PPM104}&167.404&21.679&0.135&15.0&15.937&1.536&7.409&167.485&21.679&0.135\\&167.884&21.557&0.135&10.0&17.636&0.948&2.823&167.876&21.592&0.135\\\hline
\multirow{2}{*}{PPM105*}&168.417&47.477&0.112&44.0&85.587&0.812&2.073&168.442&47.467&0.112\\&169.06&46.955&0.112&12.0&36.35&0.519&0.848&169.061&46.958&0.112\\\hline
\multirow{2}{*}{PPM106}&168.829&53.722&0.105&15.0&48.837&0.498&0.779&168.835&53.714&0.105\\&170.148&53.708&0.104&78.0&127.455&1.006&3.177&170.117&53.703&0.104\\\hline
\multirow{2}{*}{PPM107*}&170.265&34.409&0.035&11.0&26.917&0.274&0.235&170.264&34.373&0.035\\&171.577&35.34&0.035&17.0&65.468&0.174&0.095&171.601&35.345&0.035\\\hline
\multirow{3}{*}{PPM108}&170.85&19.613&0.104&56.0&61.406&1.306&5.356&170.882&19.62&0.104\\&171.581&19.244&0.103&13.0&19.616&0.935&2.747&171.63&19.252&0.103\\&171.621&19.204&0.103&26.0&21.353&1.679&8.856&171.694&19.241&0.103\\\hline
\multirow{2}{*}{PPM109}&171.464&25.513&0.114&13.0&33.373&0.708&1.575&171.47&25.538&0.114\\&171.846&25.305&0.114&23.0&46.036&0.916&2.637&171.874&25.304&0.114\\\hline
\multirow{3}{*}{PPM110*}&172.288&54.126&0.069&41.0&90.143&0.465&0.679&172.342&54.146&0.069\\&172.546&54.022&0.07&18.0&53.275&0.349&0.383&172.569&54.028&0.07\\&173.609&54.187&0.07&15.0&44.439&0.348&0.381&173.618&54.171&0.07\\\hline
\multirow{3}{*}{PPM111}&172.573&16.183&0.081&15.0&27.675&0.687&1.482&172.58&16.182&0.081\\&172.811&16.56&0.081&27.0&37.071&0.923&2.679&172.737&16.568&0.081\\&172.816&15.433&0.081&27.0&23.071&1.446&6.564&172.787&15.489&0.081\\\hline
\multirow{2}{*}{PPM112}&173.067&55.984&0.055&63.0&107.145&0.47&0.695&173.08&55.985&0.055\\&174.038&55.023&0.056&69.0&101.446&0.548&0.943&174.053&55.016&0.056\\\hline
\multirow{2}{*}{PPM113*}&173.933&40.849&0.184&28.0&148.147&0.794&1.978&173.939&40.847&0.184\\&173.969&41.312&0.183&10.0&28.043&1.472&6.807&173.951&41.323&0.183\\\hline
\multirow{2}{*}{PPM114*}&174.066&54.982&0.074&12.0&32.214&0.425&0.568&174.093&55.004&0.074\\&175.034&54.968&0.075&13.0&52.057&0.293&0.269&175.034&54.992&0.075\\\hline
\multirow{2}{*}{PPM115}&174.19&16.521&0.069&10.0&32.845&0.316&0.314&174.2&16.487&0.069\\&174.262&15.915&0.068&16.0&38.684&0.416&0.544&174.261&15.906&0.068\\\hline
\multirow{3}{*}{PPM116}&174.226&19.948&0.021&10.0&32.824&0.111&0.039&174.229&19.933&0.021\\&176.079&19.937&0.021&142.0&93.49&0.549&0.946&176.094&19.871&0.021\\&178.286&20.659&0.022&37.0&45.977&0.294&0.271&178.266&20.657&0.022\\\hline
\multirow{4}{*}{PPM117}&174.997&55.058&0.058&19.0&26.007&0.586&1.081&174.948&55.043&0.058\\&175.859&54.937&0.059&11.0&39.728&0.231&0.167&175.849&54.941&0.059\\&177.048&54.668&0.06&58.0&82.349&0.595&1.113&177.084&54.663&0.06\\&177.565&53.657&0.06&16.0&32.847&0.416&0.543&177.56&53.644&0.06\\\hline
\multirow{2}{*}{PPM118}&175.141&10.381&0.105&31.0&63.963&0.586&1.079&175.134&10.37&0.105\\&175.286&10.74&0.105&12.0&45.106&0.323&0.327&175.302&10.738&0.105\\\hline
\multirow{2}{*}{PPM119}&175.236&23.048&0.05&12.0&30.755&0.377&0.447&175.242&23.023&0.05\\&176.146&23.112&0.049&10.0&50.587&0.19&0.113&176.149&23.106&0.049\\\hline
\multirow{2}{*}{PPM120}&175.868&21.703&0.068&11.0&33.11&0.326&0.333&175.862&21.71&0.068\\&176.296&21.424&0.067&20.0&37.991&0.502&0.792&176.292&21.445&0.067\\\hline
\multirow{3}{*}{PPM121}&176.231&51.286&0.13&30.0&64.491&1.178&4.362&176.282&51.281&0.13\\&177.282&51.585&0.13&64.0&92.625&1.75&9.616&177.331&51.509&0.13\\&178.587&51.118&0.13&23.0&41.604&1.392&6.089&178.537&51.143&0.13\\\hline
\multirow{2}{*}{PPM122}&176.849&55.737&0.051&61.0&118.91&0.42&0.554&176.831&55.727&0.051\\&178.675&55.162&0.051&13.0&28.852&0.364&0.416&178.683&55.192&0.051\\\hline
\multirow{4}{*}{PPM123}&176.883&11.758&0.084&13.0&26.96&0.447&0.629&176.855&11.773&0.084\\&177.224&11.193&0.084&13.0&32.172&0.371&0.433&177.216&11.196&0.084\\&177.28&11.007&0.084&11.0&37.194&0.278&0.244&177.271&11.011&0.084\\&177.394&12.29&0.084&33.0&45.177&0.669&1.405&177.411&12.294&0.084\\\hline
\multirow{2}{*}{PPM124}&177.204&21.2&0.025&10.0&19.311&0.198&0.123&177.208&21.191&0.025\\&177.78&22.046&0.026&10.0&26.965&0.147&0.068&177.79&22.034&0.026\\\hline
\multirow{2}{*}{PPM125*}&177.5&56.482&0.066&14.0&46.771&0.291&0.266&177.466&56.481&0.066\\&177.96&56.465&0.066&10.0&26.686&0.359&0.404&177.945&56.484&0.066\\\hline
\multirow{2}{*}{PPM126}&179.21&21.258&0.069&14.0&30.68&0.466&0.681&179.203&21.26&0.069\\&179.81&20.682&0.068&11.0&14.377&0.741&1.726&179.814&20.706&0.068\\\hline
\multirow{2}{*}{PPM127*}&179.752&54.813&0.081&18.0&101.067&0.272&0.232&179.743&54.822&0.081\\&179.847&55.505&0.08&17.0&32.395&0.755&1.793&179.784&55.427&0.08\\\hline
\multirow{4}{*}{PPM128}&180.508&20.224&0.024&13.0&14.999&0.261&0.215&180.543&20.25&0.024\\&181.023&20.253&0.023&45.0&64.833&0.218&0.149&181.027&20.274&0.023\\&181.46&20.529&0.024&36.0&44.181&0.259&0.21&181.464&20.475&0.024\\&183.308&21.634&0.024&11.0&22.076&0.16&0.08&183.293&21.619&0.024\\\hline
\multirow{2}{*}{PPM129}&180.637&3.949&0.135&15.0&26.14&1.041&3.402&180.597&3.951&0.135\\&180.978&4.287&0.135&30.0&46.401&1.185&4.413&180.943&4.287&0.135\\\hline
\multirow{2}{*}{PPM130*}&180.845&51.716&0.062&17.0&53.802&0.307&0.296&180.84&51.721&0.062\\&181.105&52.451&0.063&12.0&17.988&0.629&1.243&181.047&52.43&0.063\\\hline
\multirow{2}{*}{PPM131}&181.914&14.853&0.079&17.0&25.001&0.547&0.94&181.88&14.874&0.079\\&182.238&14.856&0.079&11.0&27.129&0.33&0.342&182.227&14.855&0.079\\\hline
\multirow{2}{*}{PPM132}&182.024&25.283&0.022&14.0&27.849&0.153&0.073&181.995&25.303&0.022\\&183.849&23.99&0.022&16.0&32.976&0.148&0.069&183.845&23.983&0.022\\\hline
\multirow{2}{*}{PPM133*}&182.045&56.891&0.062&13.0&43.245&0.292&0.268&182.038&56.908&0.062\\&182.47&57.031&0.063&14.0&43.891&0.309&0.301&182.413&57.01&0.063\\\hline
\multirow{2}{*}{PPM134*}&183.103&30.593&0.107&12.0&34.783&0.651&1.331&183.11&30.627&0.107\\&183.611&30.237&0.107&29.0&87.03&0.632&1.255&183.615&30.23&0.107\\\hline
\multirow{2}{*}{PPM135}&184.6&5.191&0.077&12.0&21.1&0.461&0.666&184.593&5.181&0.077\\&184.774&5.255&0.078&13.0&30.585&0.348&0.38&184.756&5.256&0.078\\\hline
\multirow{2}{*}{PPM136*}&185.661&51.11&0.031&12.0&35.228&0.257&0.207&185.614&51.106&0.031\\&187.706&50.705&0.031&15.0&46.286&0.245&0.189&187.727&50.693&0.031\\\hline
\multirow{4}{*}{PPM137*}&186.182&31.982&0.061&33.0&79.95&0.439&0.606&186.196&31.991&0.061\\&186.414&31.409&0.06&12.0&39.797&0.32&0.321&186.403&31.427&0.06\\&186.559&31.02&0.06&33.0&69.655&0.502&0.792&186.586&31.008&0.06\\&186.679&31.358&0.06&11.0&35.051&0.331&0.345&186.696&31.343&0.06\\\hline
\multirow{2}{*}{PPM138}&188.678&28.106&0.099&15.0&33.044&0.861&2.331&188.703&28.079&0.099\\&188.711&28.56&0.099&14.0&35.499&0.736&1.704&188.731&28.58&0.099\\\hline
\multirow{2}{*}{PPM139}&188.907&26.541&0.022&18.0&33.426&0.164&0.084&188.884&26.539&0.022\\&194.549&27.833&0.023&560.0&225.409&0.779&1.907&194.477&27.765&0.023\\\hline
\multirow{5}{*}{PPM140}&189.433&15.269&0.072&26.0&37.254&0.635&1.267&189.401&15.277&0.072\\&189.655&17.215&0.071&24.0&39.343&0.55&0.952&189.665&17.191&0.071\\&189.794&16.422&0.071&37.0&46.173&0.724&1.649&189.777&16.432&0.071\\&189.854&15.472&0.071&25.0&38.825&0.583&1.069&189.861&15.475&0.071\\&190.007&16.655&0.071&10.0&19.628&0.455&0.65&190.019&16.685&0.071\\\hline
\multirow{2}{*}{PPM141*}&189.52&37.635&0.19&19.0&109.265&0.706&1.567&189.525&37.638&0.19\\&190.027&37.725&0.191&44.0&91.549&1.965&12.132&190.149&37.655&0.191\\\hline
\multirow{2}{*}{PPM142}&191.608&0.456&0.088&12.0&44.799&0.256&0.205&191.61&0.456&0.088\\&191.745&0.237&0.089&39.0&58.06&0.663&1.38&191.751&0.227&0.089\\\hline
\multirow{2}{*}{PPM143}&191.815&55.032&0.083&68.0&93.558&1.012&3.218&191.864&55.038&0.083\\&192.976&55.051&0.084&27.0&31.885&1.143&4.106&193.016&55.012&0.084\\\hline
\multirow{2}{*}{PPM144}&195.203&1.042&0.082&17.0&55.348&0.27&0.23&195.221&1.036&0.082\\&195.274&0.795&0.082&12.0&32.706&0.322&0.326&195.284&0.805&0.082\\\hline
\multirow{3}{*}{PPM145}&196.042&8.992&0.055&10.0&23.215&0.435&0.595&196.041&8.994&0.055\\&196.465&9.293&0.054&32.0&54.986&0.583&1.066&196.461&9.345&0.054\\&196.756&9.626&0.055&15.0&57.2&0.266&0.223&196.761&9.612&0.055\\\hline
\multirow{2}{*}{PPM146}&197.826&39.271&0.073&66.0&102.941&0.677&1.439&197.824&39.289&0.073\\&198.446&38.921&0.071&50.0&61.216&0.813&2.076&198.457&38.914&0.071\\\hline
\multirow{2}{*}{PPM147*}&198.417&57.253&0.079&10.0&28.522&0.56&0.987&198.454&57.232&0.079\\&198.848&57.684&0.078&10.0&57.304&0.275&0.238&198.811&57.681&0.078\\\hline
\multirow{2}{*}{PPM148}&198.894&9.917&0.051&15.0&36.798&0.377&0.446&198.916&9.924&0.051\\&199.005&8.565&0.051&16.0&29.264&0.499&0.782&199.018&8.606&0.051\\\hline
\multirow{2}{*}{PPM149*}&199.989&31.36&0.046&44.0&58.937&0.734&1.693&199.957&31.362&0.046\\&201.06&30.523&0.047&10.0&29.679&0.334&0.35&201.05&30.543&0.047\\\hline
\multirow{2}{*}{PPM150}&200.755&1.213&0.111&10.0&53.054&0.303&0.288&200.768&1.21&0.111\\&200.803&0.767&0.111&12.0&65.356&0.296&0.275&200.807&0.771&0.111\\\hline
\multirow{2}{*}{PPM151}&202.187&19.354&0.087&12.0&57.547&0.28&0.246&202.192&19.36&0.087\\&202.518&19.475&0.087&14.0&35.841&0.518&0.844&202.52&19.461&0.087\\\hline
\multirow{3}{*}{PPM152*}&202.311&59.098&0.072&13.0&44.097&0.346&0.377&202.299&59.098&0.072\\&202.832&58.84&0.072&10.0&36.473&0.312&0.305&202.823&58.858&0.072\\&204.019&58.863&0.072&11.0&38.046&0.336&0.354&204.014&58.861&0.072\\\hline
\multirow{2}{*}{PPM153}&202.336&11.698&0.023&27.0&52.346&0.221&0.153&202.316&11.694&0.023\\&203.713&13.807&0.023&12.0&27.249&0.187&0.11&203.662&13.809&0.023\\\hline
\multirow{2}{*}{PPM154*}&203.739&34.639&0.024&47.0&44.112&0.551&0.955&203.738&34.597&0.024\\&203.992&33.436&0.025&28.0&41.41&0.354&0.395&204.022&33.472&0.025\\\hline
\multirow{2}{*}{PPM155*}&203.772&42.616&0.061&13.0&17.996&0.633&1.259&203.762&42.574&0.061\\&204.041&42.708&0.062&14.0&47.345&0.266&0.223&204.039&42.721&0.062\\\hline
\multirow{5}{*}{PPM156*}&203.913&35.914&0.059&16.0&40.089&0.37&0.431&203.915&35.901&0.059\\&203.963&36.599&0.061&12.0&25.712&0.418&0.549&203.959&36.619&0.061\\&204.235&34.842&0.06&23.0&36.096&0.576&1.042&204.283&34.833&0.06\\&204.254&35.993&0.06&20.0&33.093&0.544&0.931&204.245&35.979&0.06\\&204.26&35.253&0.06&12.0&19.379&0.556&0.97&204.276&35.262&0.06\\\hline
\multirow{3}{*}{PPM157}&205.427&26.361&0.075&43.0&67.67&0.583&1.069&205.399&26.368&0.075\\&206.297&26.894&0.075&11.0&40.884&0.247&0.191&206.294&26.901&0.075\\&206.298&26.897&0.075&10.0&40.796&0.225&0.159&206.304&26.902&0.075\\\hline
\multirow{2}{*}{PPM158}&206.195&0.139&0.089&12.0&41.538&0.307&0.295&206.195&0.14&0.089\\&206.798&0.394&0.089&10.0&80.436&0.132&0.055&206.794&0.392&0.089\\\hline
\multirow{2}{*}{PPM159}&206.281&6.077&0.127&10.0&28.777&0.7&1.54&206.293&6.071&0.127\\&206.387&5.77&0.127&21.0&40.133&1.052&3.48&206.406&5.793&0.127\\\hline
\multirow{2}{*}{PPM160*}&207.738&46.314&0.064&11.0&35.282&0.281&0.248&207.74&46.322&0.064\\&208.071&46.402&0.063&17.0&45.978&0.336&0.355&208.052&46.406&0.063\\\hline
\multirow{2}{*}{PPM161*}&208.484&33.156&0.05&40.0&58.85&0.699&1.536&208.525&33.109&0.05\\&209.605&32.659&0.049&39.0&68.665&0.584&1.071&209.622&32.675&0.049\\\hline
\multirow{2}{*}{PPM162*}&208.91&49.466&0.106&10.0&58.375&0.324&0.331&208.932&49.454&0.106\\&209.621&49.536&0.106&46.0&139.049&0.627&1.234&209.651&49.532&0.106\\\hline
\multirow{2}{*}{PPM163}&210.107&28.536&0.063&12.0&22.65&0.427&0.572&210.108&28.536&0.063\\&210.454&28.535&0.063&13.0&21.826&0.479&0.722&210.512&28.524&0.063\\\hline
\multirow{2}{*}{PPM164*}&210.4&39.719&0.079&10.0&34.222&0.392&0.483&210.407&39.73&0.079\\&210.765&39.944&0.079&11.0&38.916&0.384&0.462&210.824&39.95&0.079\\\hline
\multirow{2}{*}{PPM165}&211.072&6.384&0.113&13.0&25.335&0.682&1.459&211.081&6.365&0.113\\&211.554&6.607&0.114&19.0&38.044&0.666&1.392&211.572&6.575&0.114\\\hline
\multirow{3}{*}{PPM166}&213.632&1.738&0.054&11.0&53.322&0.142&0.063&213.63&1.732&0.054\\&214.324&1.165&0.054&18.0&58.204&0.213&0.143&214.325&1.193&0.054\\&214.38&2.036&0.055&36.0&70.268&0.353&0.392&214.375&2.024&0.055\\\hline
\multirow{2}{*}{PPM167}&213.768&26.372&0.071&11.0&28.688&0.344&0.372&213.772&26.387&0.071\\&214.523&26.509&0.071&35.0&38.398&0.805&2.035&214.507&26.516&0.071\\\hline
\multirow{2}{*}{PPM168}&214.709&26.368&0.036&10.0&16.624&0.364&0.415&214.708&26.405&0.036\\&216.018&26.211&0.037&34.0&45.668&0.468&0.689&216.025&26.227&0.037\\\hline
\multirow{2}{*}{PPM169*}&215.401&49.541&0.071&14.0&49.97&0.269&0.227&215.405&49.545&0.071\\&215.403&49.54&0.071&15.0&49.603&0.293&0.269&215.414&49.538&0.071\\\hline
\multirow{2}{*}{PPM170*}&216.132&36.049&0.029&28.0&21.971&0.877&2.417&216.222&36.087&0.029\\&217.619&36.419&0.029&18.0&29.858&0.431&0.582&217.591&36.413&0.029\\\hline
\multirow{2}{*}{PPM171*}&216.97&57.023&0.106&10.0&18.772&0.41&0.522&216.97&57.023&0.106\\&217.135&56.802&0.106&24.0&27.115&0.67&1.408&217.135&56.802&0.106\\\hline
\multirow{2}{*}{PPM172*}&217.105&56.857&0.106&30.0&67.879&0.761&1.818&217.074&56.871&0.106\\&217.741&57.406&0.106&27.0&96.098&0.48&0.723&217.693&57.405&0.106\\\hline
\multirow{4}{*}{PPM173}&217.703&25.648&0.096&50.0&56.154&1.384&6.02&217.686&25.64&0.096\\&218.072&26.021&0.094&13.0&34.239&0.505&0.802&218.088&26.006&0.094\\&218.614&26.325&0.095&10.0&36.666&0.364&0.416&218.611&26.318&0.095\\&218.616&26.334&0.095&11.0&33.869&0.432&0.587&218.628&26.322&0.095\\\hline
\multirow{2}{*}{PPM174}&218.432&18.824&0.076&17.0&42.456&0.401&0.504&218.414&18.806&0.076\\&218.537&18.535&0.077&11.0&24.009&0.466&0.681&218.535&18.557&0.077\\\hline
\multirow{2}{*}{PPM175*}&218.62&54.808&0.14&19.0&84.764&0.572&1.03&218.642&54.806&0.14\\&218.841&55.191&0.139&40.0&98.636&1.019&3.264&218.798&55.2&0.139\\\hline
\multirow{3}{*}{PPM176}&218.933&17.896&0.049&10.0&27.379&0.279&0.245&218.936&17.887&0.049\\&219.222&18.395&0.049&12.0&49.643&0.186&0.109&219.236&18.405&0.049\\&219.611&17.653&0.048&16.0&33.281&0.369&0.427&219.624&17.673&0.048\\\hline
\multirow{2}{*}{PPM177*}&219.434&30.423&0.159&11.0&22.76&1.298&5.295&219.371&30.443&0.159\\&220.292&30.173&0.159&11.0&12.3&2.298&16.594&220.296&30.214&0.159\\\hline
\multirow{3}{*}{PPM178}&220.471&13.321&0.121&26.0&76.913&0.487&0.746&220.474&13.332&0.121\\&220.586&12.93&0.122&14.0&32.936&0.618&1.199&220.577&12.932&0.122\\&220.924&13.205&0.122&12.0&25.072&0.685&1.472&220.934&13.198&0.122\\\hline
\multirow{2}{*}{PPM179}&220.56&22.303&0.097&26.0&41.008&0.839&2.21&220.552&22.277&0.097\\&221.081&22.303&0.096&10.0&26.449&0.5&0.786&221.072&22.291&0.096\\\hline
\multirow{2}{*}{PPM180*}&220.645&31.276&0.063&12.0&31.802&0.415&0.542&220.655&31.295&0.063\\&220.924&31.557&0.063&13.0&32.885&0.435&0.594&220.939&31.552&0.063\\\hline
\multirow{2}{*}{PPM181*}&221.505&46.214&0.086&13.0&32.76&0.708&1.576&221.469&46.222&0.086\\&221.956&46.466&0.086&11.0&33.863&0.601&1.133&221.953&46.45&0.086\\\hline
\multirow{2}{*}{PPM182}&221.77&11.592&0.029&11.0&42.456&0.118&0.044&221.761&11.583&0.029\\&221.785&13.624&0.03&48.0&54.754&0.411&0.531&221.802&13.586&0.03\\\hline
\multirow{3}{*}{PPM183}&222.941&22.566&0.117&30.0&46.35&0.932&2.731&222.921&22.561&0.117\\&222.959&22.552&0.117&22.0&40.827&0.774&1.884&222.956&22.545&0.117\\&223.359&21.968&0.117&50.0&60.922&1.296&5.279&223.351&21.965&0.117\\\hline
\multirow{4}{*}{PPM184}&223.314&18.125&0.059&14.0&25.192&0.428&0.577&223.319&18.139&0.059\\&223.39&18.097&0.059&10.0&30.5&0.257&0.207&223.365&18.099&0.059\\&223.927&19.28&0.059&13.0&21.573&0.462&0.669&223.955&19.241&0.059\\&223.963&19.281&0.059&15.0&24.859&0.464&0.676&223.96&19.26&0.059\\\hline
\multirow{2}{*}{PPM185*}&224.011&47.451&0.086&12.0&66.309&0.34&0.363&223.992&47.454&0.086\\&224.649&47.422&0.086&39.0&85.708&0.846&2.25&224.678&47.438&0.086\\\hline
\multirow{2}{*}{PPM186*}&224.644&47.521&0.088&12.0&48.721&0.249&0.195&224.644&47.521&0.088\\&225.311&47.261&0.088&37.0&56.021&0.736&1.704&225.311&47.261&0.088\\\hline
\multirow{2}{*}{PPM187}&225.782&7.979&0.089&15.0&51.971&0.316&0.314&225.789&7.991&0.089\\&225.907&7.819&0.088&11.0&48.347&0.247&0.192&225.914&7.807&0.088\\\hline
\multirow{2}{*}{PPM188}&227.029&16.582&0.118&21.0&52.973&0.643&1.297&227.039&16.593&0.118\\&227.348&16.313&0.118&16.0&30.754&0.835&2.19&227.342&16.325&0.118\\\hline
\multirow{3}{*}{PPM189*}&227.299&52.522&0.012&11.0&44.222&0.102&0.033&227.215&52.498&0.012\\&228.79&55.518&0.011&12.0&30.886&0.155&0.075&228.785&55.54&0.011\\&233.501&56.686&0.011&10.0&32.229&0.121&0.046&233.574&56.645&0.011\\\hline
\multirow{2}{*}{PPM190}&227.702&5.948&0.078&11.0&40.146&0.225&0.158&227.692&5.946&0.078\\&227.732&5.78&0.079&40.0&76.215&0.438&0.602&227.728&5.767&0.079\\\hline
\multirow{2}{*}{PPM191}&227.773&5.315&0.081&19.0&64.828&0.259&0.21&227.776&5.312&0.081\\&227.873&6.282&0.08&39.0&54.951&0.615&1.188&227.87&6.267&0.08\\\hline
\multirow{2}{*}{PPM192}&228.804&4.555&0.098&10.0&34.282&0.349&0.382&228.81&4.559&0.098\\&228.842&4.374&0.097&33.0&84.083&0.468&0.688&228.847&4.36&0.097\\\hline
\multirow{2}{*}{PPM193*}&229.019&45.223&0.063&10.0&36.46&0.318&0.319&228.996&45.224&0.063\\&229.803&45.062&0.064&24.0&56.505&0.483&0.732&229.875&45.087&0.064\\\hline
\multirow{2}{*}{PPM194}&229.846&20.815&0.04&45.0&72.146&0.397&0.496&229.853&20.811&0.04\\&231.089&20.757&0.04&32.0&64.444&0.316&0.314&231.089&20.757&0.04\\\hline
\multirow{2}{*}{PPM195*}&230.848&31.056&0.074&35.0&40.454&0.845&2.242&230.902&31.02&0.074\\&230.932&31.172&0.075&10.0&21.93&0.457&0.657&230.924&31.175&0.075\\\hline
\multirow{2}{*}{PPM196}&231.484&29.83&0.114&24.0&54.781&0.695&1.515&231.493&29.815&0.114\\&231.637&29.688&0.114&47.0&43.49&1.686&8.93&231.679&29.709&0.114\\\hline
\multirow{2}{*}{PPM197}&231.781&28.347&0.066&10.0&29.023&0.331&0.345&231.785&28.352&0.066\\&231.897&28.801&0.066&65.0&68.827&0.904&2.569&231.934&28.799&0.066\\\hline
\multirow{2}{*}{PPM198}&232.153&28.29&0.073&12.0&39.255&0.274&0.236&232.16&28.288&0.073\\&233.189&28.043&0.073&42.0&48.852&0.762&1.826&233.182&28.032&0.073\\\hline
\multirow{3}{*}{PPM199}&232.451&29.015&0.085&18.0&41.086&0.415&0.542&232.465&29.01&0.085\\&232.468&29.027&0.085&16.0&41.971&0.362&0.411&232.468&29.025&0.085\\&232.848&28.988&0.084&13.0&35.524&0.342&0.366&232.833&28.985&0.084\\\hline
\multirow{2}{*}{PPM200*}&232.452&42.734&0.019&10.0&54.986&0.14&0.061&232.483&42.75&0.019\\&234.13&43.438&0.019&20.0&92.469&0.173&0.094&234.136&43.459&0.019\\\hline
\multirow{2}{*}{PPM201*}&235.648&41.823&0.142&24.0&70.612&0.919&2.655&235.649&41.844&0.142\\&236.169&41.503&0.142&13.0&33.015&1.058&3.514&236.148&41.551&0.142\\\hline
\multirow{2}{*}{PPM202}&235.805&36.371&0.065&11.0&26.654&0.381&0.456&235.827&36.371&0.065\\&236.233&36.11&0.066&50.0&125.395&0.379&0.452&236.222&36.102&0.066\\\hline
\multirow{2}{*}{PPM203}&236.615&3.432&0.096&19.0&61.51&0.362&0.411&236.62&3.44&0.096\\&236.705&3.266&0.096&19.0&104.199&0.211&0.14&236.705&3.268&0.096\\\hline
\multirow{4}{*}{PPM204*}&237.409&41.983&0.034&19.0&34.597&0.405&0.515&237.303&42.004&0.034\\&238.728&41.536&0.034&40.0&66.752&0.441&0.61&238.759&41.547&0.034\\&238.751&39.75&0.033&15.0&53.564&0.206&0.133&238.792&39.741&0.033\\&239.121&41.905&0.035&18.0&46.407&0.29&0.265&239.042&41.91&0.035\\\hline
\multirow{4}{*}{PPM205}&238.848&28.993&0.078&23.0&51.188&0.398&0.499&238.859&29.012&0.078\\&238.898&28.85&0.077&11.0&26.625&0.364&0.416&238.922&28.84&0.077\\&239.189&28.657&0.078&22.0&33.37&0.579&1.052&239.177&28.64&0.078\\&239.48&28.8&0.076&30.0&65.283&0.408&0.523&239.473&28.8&0.076\\\hline
\multirow{2}{*}{PPM206*}&239.384&35.575&0.159&20.0&36.201&1.419&6.329&239.376&35.624&0.159\\&239.905&35.331&0.159&10.0&21.81&1.208&4.585&239.859&35.349&0.159\\\hline
\multirow{6}{*}{PPM207*}&241.324&53.207&0.063&12.0&40.897&0.436&0.598&241.283&53.194&0.063\\&242.404&53.052&0.063&18.0&95.195&0.283&0.251&242.399&53.056&0.063\\&242.548&53.74&0.064&31.0&52.631&0.899&2.541&242.505&53.674&0.064\\&242.718&52.456&0.063&25.0&81.36&0.45&0.636&242.746&52.476&0.063\\&242.771&52.802&0.064&14.0&46.419&0.456&0.654&242.79&52.818&0.064\\&243.8&52.583&0.062&10.0&48.282&0.296&0.274&243.77&52.587&0.062\\\hline
\multirow{6}{*}{PPM208*}&245.75&37.88&0.031&16.0&35.21&0.201&0.127&245.741&37.891&0.031\\&246.888&42.679&0.031&10.0&26.285&0.168&0.089&246.895&42.678&0.031\\&247.084&40.896&0.032&17.0&42.541&0.177&0.099&247.109&40.884&0.032\\&247.546&40.722&0.029&49.0&69.835&0.32&0.323&247.537&40.739&0.029\\&247.827&39.795&0.03&16.0&39.155&0.185&0.108&247.82&39.83&0.03\\&247.83&39.797&0.03&17.0&38.727&0.199&0.125&247.824&39.839&0.03\\\hline
\multirow{2}{*}{PPM209*}&246.921&40.966&0.032&10.0&33.479&0.133&0.055&246.911&40.945&0.032\\&247.301&40.611&0.031&12.0&38.055&0.14&0.062&247.307&40.608&0.031\\\hline
\multirow{4}{*}{PPM210*}&257.805&63.652&0.08&10.0&56.285&0.195&0.119&257.833&63.643&0.08\\&258.779&64.042&0.081&10.0&68.719&0.16&0.08&258.798&64.037&0.081\\&259.037&63.945&0.081&11.0&53.999&0.223&0.157&259.006&63.923&0.081\\&261.179&64.279&0.081&19.0&52.46&0.396&0.492&261.137&64.289&0.081\\\hline
\multirow{2}{*}{PPM211*}&262.321&54.243&0.081&23.0&244.824&0.201&0.127&262.334&54.234&0.081\\&262.35&54.485&0.081&22.0&286.826&0.163&0.084&262.356&54.478&0.081\\\hline
\multirow{2}{*}{PPM212}&314.227&0.179&0.048&12.0&182.426&0.165&0.085&314.223&0.165&0.048\\&314.652&0.936&0.048&16.0&84.88&0.465&0.68&314.648&0.924&0.048\\\hline
\multirow{2}{*}{PPM213}&319.913&0.688&0.035&10.0&61.46&0.221&0.153&319.913&0.675&0.034\\&320.311&1.087&0.035&20.0&63.294&0.427&0.573&320.342&1.076&0.035\\\hline
\multirow{2}{*}{PPM214}&320.094&0.495&0.135&13.0&40.585&0.685&1.476&320.092&0.47&0.135\\&320.477&0.523&0.135&10.0&48.236&0.443&0.618&320.493&0.523&0.135\\\hline
\multirow{2}{*}{PPM215}&320.934&0.874&0.139&21.0&33.338&1.546&7.511&320.93&0.864&0.139\\&321.008&0.884&0.141&16.0&37.196&1.161&4.233&321.0&0.885&0.141\\\hline
\multirow{4}{*}{PPM216}&321.105&1.065&0.05&27.0&78.323&0.489&0.751&321.091&1.055&0.05\\&321.904&0.974&0.049&18.0&53.891&0.458&0.66&321.871&0.957&0.049\\&322.143&1.229&0.049&12.0&117.016&0.145&0.066&322.151&1.217&0.049\\&322.62&0.858&0.05&20.0&42.985&0.66&1.371&322.63&0.86&0.05\\\hline
\multirow{3}{*}{PPM217}&333.15&13.968&0.027&25.0&75.547&0.276&0.239&333.152&13.983&0.027\\&333.923&13.742&0.026&12.0&62.527&0.158&0.079&333.92&13.743&0.026\\&333.926&13.77&0.026&18.0&67.04&0.222&0.155&333.944&13.767&0.026\\\hline
\multirow{2}{*}{PPM218}&337.038&0.58&0.059&13.0&70.029&0.244&0.187&337.011&0.586&0.059\\&337.27&0.126&0.058&26.0&137.461&0.249&0.195&337.274&0.119&0.058\\\hline
\multirow{2}{*}{PPM219}&338.131&0.767&0.059&25.0&52.374&0.624&1.225&338.169&0.782&0.059\\&338.892&1.13&0.059&23.0&70.737&0.427&0.572&338.902&1.144&0.059\\\hline
\multirow{2}{*}{PPM220}&339.025&13.01&0.089&14.0&70.38&0.289&0.262&339.032&13.02&0.089\\&339.245&13.244&0.089&30.0&121.818&0.364&0.416&339.247&13.251&0.089\\\hline
\multirow{2}{*}{PPM221}&339.65&0.075&0.059&10.0&72.435&0.182&0.104&339.645&0.076&0.059\\&340.661&1.123&0.058&13.0&51.983&0.329&0.339&340.674&1.112&0.058\\\hline

